Generalized Batch Normalization: Towards Accelerating Deep Neural Networks

Utilizing recently introduced concepts from statistics and quantitative risk management, we present a general variant of Batch Normalization (BN) that offers accelerated convergence of Neural Network training compared to conventional BN. In general, we show that mean and standard deviation are not always the most appropriate choice for the centering and scaling procedure within the BN transformation, particularly if ReLU follows the normalization step. We present a Generalized Batch Normalization (GBN) transformation, which can utilize a variety of alternative deviation measures for scaling and statistics for centering, choices which naturally arise from the theory of generalized deviation measures and risk theory in general. When used in conjunction with the ReLU non-linearity, the underlying risk theory suggests natural, arguably optimal choices for the deviation measure and statistic. Utilizing the suggested deviation measure and statistic, we show experimentally that training is accelerated more so than with conventional BN, often with improved error rate as well. Overall, we propose a more flexible BN transformation supported by a complimentary theoretical framework that can potentially guide design choices.

==> experiments2.tex <==
\subsection{CIFAR-10, CIFAR-100, and SVHN}
We compare the performance and convergence rate on the CIFAR-10, CIFAR-100, and Street View House Numbers (SVHN) datasets. The CIFAR-10 and CIFAR-100 dataset consist of 60,000 tiny color images (32x32) with 10 and 100 classes for image recognition task respectively~\cite{krizhevsky2009learning}. The SVHN Dataset consists of Google Street View images with 10 house digit classes~\cite{netzer2011reading}. 

We trained LeNet networks on the CIFAR-10 (200 epochs) and the SVHN (200 epochs) datasets. The setting is set similar to that used with MNIST dataset: SGD with learning rate 0.1 and 0.01, batch size 1024.
Figure~\ref{fig:cifar10} and Figure~\ref{fig:svhn} illustrate the performance comparison of six different choices of deviation measure on the CIFAR-10 and SVHN datasets respectively. 

We also train a ResNet architecture with 20 layers (exactly same architecture and settings used in~\cite{he2015delving}) for 200 epochs on the CIFAR-10 and CIFAR-100 dataset.
We trained the ResNet with and without data augmentation (i.e., random crop and random horizontal flip). For the CIFAR-10 dataset, we observe that with data augmentation, the proposed methods achieve the similar performance as standard BN. However, if we do not augment data (less symmetric distribution), both RSD and MAD perform better than standard BN (Figure~\ref{fig:cifar10-resnet}). For the CIFAR-100 dataset, even with data augmentation, RSD and MAN outperform standard BN (Figure~\ref{fig:cifar100-resnet}).

\begin{table*}[!tb]
\centering
\small
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Dataset  & Architecture & Learning Rate & Batch Size & SD    & MAD   & RSD   & RBD   & SQD1  & SQD2  & SQD3  \\ \hline
CIFAR-10 & LeNet        & 0.1           & 256        & 30.73 & 29.70 & 30.04 & 30.38 & 33.29 & 29.53 & \textbf{29.07} \\ \hline
CIFAR-10 & LeNet        & 0.1           & 1024       & 29.31 & 28.58 & 28.85 & 31.05 & 33.33 & 28.63 & \textbf{28.03} \\ \hline
CIFAR-10 & LeNet        & 0.1           & 2048       & 28.96 & 29.32 & \textbf{27.51} & 36.28 & 39.94 & 28.79 & 29.18 \\ \hline
CIFAR-10 & LeNet        & 0.01          & 256        & 29.69 & 29.03 & 29.90 & 33.32 & 29.99 & 27.96 & \textbf{27.36} \\ \hline
CIFAR-10 & LeNet        & 0.01          & 1024       & \textbf{28.29} & 28.37 & 29.44 & 47.51 & 30.62 & 29.33 & 30.97 \\ \hline
CIFAR-10 & LeNet        & 0.01          & 2048       & 31.64 & \textbf{30.53} & 30.81 & 57.08 & 32.45 & 31.35 & 37.26 \\ \hline
CIFAR-10 & ResNet20     & 0.1           & 1024       & 29.67 & 29.33 & 30.55 & \textbf{20.49} & 23.64 & 24.86 & 24.99 \\ \hline
CIFAR-10 & ResNet20     & 0.01          & 1024       & 34.57 & 33.59 & 35.52 & 47.17 & 32.20 & \textbf{32.02} & 47.89 \\ \hline
SVHN     & LeNet        & 0.1           & 1024       & 10.68 & 10.17 & 10.91 & 12.17 & 80.41 & 10.60 & \textbf{10.08} \\ \hline
SVHN     & LeNet        & 0.1           & 2048       & 10.46 & 10.18 & 10.57 & 13.58 & 22.03 & 10.68 & \textbf{9.75}  \\ \hline
SVHN     & LeNet        & 0.01          & 1024       & 10.83 & 10.46 & \textbf{10.30} & 20.62 & 11.62 & 10.87 & 11.29 \\ \hline
SVHN     & LeNet        & 0.01          & 2048       & 12.60 & 11.74 & \textbf{11.22} & 43.04 & 11.99 & 11.83 & 12.80 \\ \hline
\end{tabular}
\caption{Performance Comparison of Error Rate (\%)) on the CIFAR-10 and SVHN datasets.}
\label{tab:cifar10-svhn}
\end{table*}

\begin{figure}[!htb]
% \vskip 0.2in
\begin{center}
\begin{subfigure}[b]{0.48\columnwidth}
\centering
\includegraphics[width=\columnwidth]{figs/cifar10-lenet-lr0_01-1024_train_loss.pdf}
\caption{\scriptsize{Training Loss}}
\end{subfigure}
\begin{subfigure}[b]{0.48\columnwidth}
\centering
\includegraphics[width=\columnwidth]{figs/cifar10-lenet-lr0_01-1024_test_err.pdf}
\caption{\scriptsize{Test Error Rate}}
\end{subfigure}
\caption{Performance comparison on the CIFAR-10 dataset using LeNet. X-axis: Number of epochs; Y-axis: Training loss/Test error rate (\%).}
\label{fig:cifar10}
\end{center}

\end{figure}
\begin{figure}[!htb]
\begin{center}
\begin{subfigure}[b]{0.48\columnwidth}
\centering
\includegraphics[width=\columnwidth]{figs/svhn-lenet-lr0_01-1024_train_loss.pdf}
\caption{\scriptsize{Training Loss}}
\end{subfigure}
\begin{subfigure}[b]{0.48\columnwidth}
\centering
\includegraphics[width=\columnwidth]{figs/svhn-lenet-lr0_01-1024_test_err.pdf}
\caption{\scriptsize{Test Error Rate}}
\end{subfigure}
\caption{Performance comparison on the SVHN dataset. X-axis: Number of epochs; Y-axis: Training loss/Test error rate (\%).}
\label{fig:svhn}
\end{center}
\end{figure}

\begin{figure}[!htb]
\begin{center}
\begin{subfigure}[b]{0.48\columnwidth}
\centering
\includegraphics[width=\columnwidth]{figs/cifar10-resnet-lr-0_01-bs-1024_train_loss.pdf}
\caption{\scriptsize{Training Loss}}
\end{subfigure}
\begin{subfigure}[b]{0.48\columnwidth}
\centering
\includegraphics[width=\columnwidth]{figs/cifar10-resnet-lr-0_01-bs-1024_test_err.pdf}
\caption{\scriptsize{Test Error Rate}}
\end{subfigure}
\caption{Performance comparison on the CIFAR-10 dataset using ResNet20. X-axis: Number of epochs; Y-axis: Training loss/Test error rate (\%).}
\label{fig:cifar10-resnet}
\end{center}
\end{figure}

\begin{figure}[!htb]
\begin{center}
\begin{subfigure}[b]{0.48\columnwidth}
\centering
\includegraphics[width=\columnwidth]{figs/cifar100_resnet18_train_loss.pdf}
\caption{\scriptsize{Training Loss}}
\end{subfigure}
\begin{subfigure}[b]{0.48\columnwidth}
\centering
\includegraphics[width=\columnwidth]{figs/cifar100_resnet18_test_err.pdf}
\caption{\scriptsize{Test Error Rate}}
\end{subfigure}
\caption{Performance comparison on the CIFAR-100 dataset using ResNet20. X-axis: Number of epochs; Y-axis: Training loss/Test error rate (\%).}
\label{fig:cifar100-resnet}
\end{center}
\end{figure}
\newpage
Most methods (MAD, SQD1, SQD2, and RSD) converge faster than standard SD. The error rates of these methods are similar, but with slight improvement achieved by the proposed alternative deviation measures. Table~\ref{tab:cifar10-svhn} contains more detailed results, including the best error rate achieved for a few extra settings. However, faster converting alternatives achieve similar error rates. Here, we see that not only can faster convergence be achieved with alternative deviation measures, but increased accuracy as well.



% \subsection{UCI}
% We conduct experiments on 111 UCI Machine Learning Repository datasets following~\cite{klambauer2017self}. We retrieved classification datasets from the UCI Machine Learning repository. We removed the datasets where the number of data samples is larger than 1000, then separated them into ``small'' and ``large'' datasets. The ``small'' datasets are datasets with less than 1000 data samples, while the ``large'' datasets consist more than 1000 data samples. Detailed information on features and size of the UCI datasets is discussed in~\cite{klambauer2017self}.

% We train a neural network with fully connected layers, batch normalization, and ReLU activation. We perform a grid search on these datasets with different hyper-parameters: 1) learning rate 0.1 and 0.01; 2) batch size 512 and 1024; 3) number of layers 2, 4, 8, and 16; 4) number of hidden units 256 and 512. Early stopping is adopted when the validation loss cannot improve within 10 epochs. We select the best models using grid searching and evaluated them on the test dataset. 

% Figure~\ref{fig:uci} shows the performance comparison on the UCI datasets. For this figure, we first measure the convergence rate of each method on each dataset via (accuracy/\#epochs). We then declare the `winner' to be the method with best convergence rate. In Figure~\ref{fig:uci}, the line plots the number of `wins' for each method over the entire UCI dataset. To compare accuracy, we report average accuracy over all datasets. The bar plots the average accuracy.
% \begin{figure}[!htb]
% \centering
% \begin{subfigure}[b]{0.75\columnwidth}
% \centering
% \includegraphics[width=\columnwidth]{figs/uci_small.png}
% \end{subfigure}

% \begin{subfigure}[b]{0.75\columnwidth}
% \centering
% \includegraphics[width=\columnwidth]{figs/uci_big.png}
% \end{subfigure}
% \vskip -0.2in

% \caption{Performance comparison on the UCI datasets. The top figure shows the results on the ``small'' datasets. The bottom figure shows the results on the ``large'' datasets. Bars indicate the average accuracy over all the UCI datasets. Line indicate the number of convergence rate `wins.', which is calculated by $\frac{accuracy}{\#epochs}$ }
% \label{fig:uci}
% \vskip -0.3in
% \end{figure}

% The performance and convergence rate of SD performs the best on the ``small'' datasets. However, on the ``large'' datasets, RSD converges faster and achieves better accuracy than SD. SQD1 also has comparable performance and convergence rate.


